Mathematical meal models for simulation of human metabolism

We present and critically discuss five commonly used mathematical models of the meal glucose rate of appearance in humans. Such models are key to simulation of the metabolism in healthy people, people with diabetes, and obese people, and they are central to developing effective treatments and prevention strategies. Furthermore, we discuss important aspects of systematic mathematical modeling of human metabolism, including meal consumption modeling, stoichiometry and reaction kinetics, and general-purpose model components.

==> fig/tikz/pfr_diagram.tex <==
\begin{tikzpicture}
    \node[cylinder, minimum width=40pt, minimum height=200pt, draw] (c) at (0,0) {$v \rightarrow$};
\end{tikzpicture}
